InspectorRAGet: An Introspection Platform for RAG Evaluation

Large Language Models (LLM) have become a popular approach for implementing Retrieval Augmented Generation (RAG) systems, and a significant amount of effort has been spent on building good models and metrics. In spite of increased recognition of the need for rigorous evaluation of RAG systems, few tools exist that go beyond the creation of model output and automatic calculation. We present InspectorRAGet, an introspection platform for performing a comprehensive analysis of the quality of RAG system output. InspectorRAGet allows the user to analyze aggregate and instance-level performance of RAG systems, using both human and algorithmic metrics as well as annotator quality. InspectorRAGet is suitable for multiple use cases and is available publicly to the community. A live instance of the platform is available at https://ibm.biz/InspectorRAGet.

==> use-case-screenshots.tex <==
\section{Use Case Screenshots}
\label{app:screenshots}

We provide screenshots showcasing several of the findings we describe in Section~\ref{sec:insights} in Figures~\ref{fig:longnq_prediction}-\ref{fig:mt_length}.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/longnq_predictions.png}
    \caption{Predictions View: Prediction Example from \datasetname. This highlights an example of Llama starting with ``Sure, I'd be happy to help!"}
    \label{fig:longnq_prediction}
\end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/longnq_algo_overview.png}
    \caption{Performance Overview: Algorithmic Metrics Overview of \datasetname. Compare with Human Metrics Overview in Figure~\ref{fig:longnq_human_overview}}
    \label{fig:longnq_alg_overview}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/longnq_human_overview.png}
    \caption{Performance Overview: Human Metrics Overview of \datasetname. This highlights that Llama is preferred least by humans. It also shows that humans rank Mistral answers higher than algorithmic metrics (Figure~\ref{fig:longnq_alg_overview}) }
    \label{fig:longnq_human_overview}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/longnq_ext_vs_faithful.png}
    \caption{Metric Behavior: The majority of instances receive high scores for both Extractiveness and Faithfulness in \datasetname.}
    \label{fig:extractive_vs_faithful}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/longnq_win_agreement.png}
    \caption{Annotator Behavior: Agreement for \datasetname\ on model outputs. Unexepectedly, disagreement between annotators with regard to reference responses are similar to those of generated responses.}
    \label{fig:longnq_agreement}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/longnq_low_relevance.png}
    \caption{Model Behavior: Low Agreement on Answer Relevance for reference responses of \datasetname.}
    \label{fig:low_relevance}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/longnq_llama_extractive.png}
    \caption{Model Comparator: Llama is significantly more extractive than GPT 3.5 for \datasetname.}
    \label{fig:llama_extractive}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/longnq_hardquestion.png}
    \caption{Detailed View: Example of a question that is hard to interpret from \datasetname{} leading to disagreement among annotators with regard to answer relevance.}
    \label{fig:hard_question}
\end{figure*}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/mt_annotators.png}
    \caption{Annotator Behavior: The human annotators (Experts) tend to agree on head-to-head winner for MT-Bench.}
    \label{fig:mt_agreement}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/mt_winner.png}
    \caption{Model Behavior: GPT-4 responses win the most according to experts and GPT-4-judge. The experts and GPT-4-judge yield a very similar winning model distribution. They differ mostly in choosing GPT-4 as a winner (self-enhancement bias of GPT-4-judge) and declaring ties.}
    \label{fig:mt_win}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/mt_position.png}
    \caption{Model Behavior: while position distribution seem to be quite uniform among experts, GPT-4 was presented with models responses in a biased manner, with some models always occurring in the first or second position.}
    \label{fig:mt_position}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/mt_length.png}
    \caption{Model Behavior: There is a verbosity bias. Alpaca-13B and LLama-13B answers are the shortest and they lose the most as shown in Figure~\ref{fig:mt_win}.}
    \label{fig:mt_length}
\end{figure}
